MLBench: How Good Are Machine Learning Clouds for Binary Classification Tasks on Structured Data?

We conduct an empirical study of machine learning functionalities provided by major cloud service providers, which we call machine learning clouds. Machine learning clouds hold the promise of hiding all the sophistication of running large-scale machine learning: Instead of specifying how to run a machine learning task, users only specify what machine learning task to run and the cloud figures out the rest. Raising the level of abstraction, however, rarely comes free - a performance penalty is possible. How good, then, are current machine learning clouds on real-world machine learning workloads? We study this question with a focus on binary classication problems. We present mlbench, a novel benchmark constructed by harvesting datasets from Kaggle competitions. We then compare the performance of the top winning code available from Kaggle with that of running machine learning clouds from both Azure and Amazon on mlbench. Our comparative study reveals the strength and weakness of existing machine learning clouds and points out potential future directions for improvement.

==> %5BEDBT 2018%5D SoMLC 2/backup.tex <==
%\vspace{-1em}
\section{Backup}

\paragraph*{Premier of Clouds APIs} 

\vspace{-1em}
\paragraph*{Summary of Insights} Our
study is organized with the following
structure. We mainly focus on three aspects
of machine learning clouds: (1) {\em Is
the set of machine learning models
enough?} (2) {\em Is the performance of 
training enough?} and (3) {\em Is the hyperparameter
tuning support enough?} For each 
level of error tolerances and budget
of time and money, we discuss 
each of these three questions for
each of the two machine learning. In
this paper, we fully studied this 
``cross product'' and highlight some
interesting insights here.\\

\vspace{-0.5em}
\noindent
{\bf (Low Tolerance Regime)} 
This regime corresponds to
the case when the error tolerance from the user
is low --- for example, when users can only be
satisfied by winning the Kaggle competition
or being ranked among the top 1\%.
Our study reveals the following:
\begin{enumerate}
    \vspace{-0.25em}
    \item {\bf Even with the same features
    engineered by the winning Kaggle entry, 
    neither Azure nor Amazon is able to meet  
    the tolerance for {\em all} datasets.}
    The fundamental reason is that both clouds
    miss ensemble-based models in their API.
    \item {\bf ?????}
\end{enumerate}

\noindent
{\bf (High Tolerance Regime)}
This regime corresponds to
the case when the error tolerance from the user
is high --- for example, when users are 
happy with suboptimal quality that is only
up to 5 points lower than the winning Kaggle
entry or being ranked among the top 10\%.
Our study reveals the following:
\begin{enumerate}
    \vspace{-0.25em}
    \item {\bf With the same features
    engineered by the winning Kaggle entry,
    both Azure and Amazon are able to meet
    the tolerance for {\em most} datasets.}
    For example, the default setting of Amazon 
    can already provide enough quality for this case.
    \vspace{-0.25em}
    \item {\bf With the same features
    engineered by the winning Kaggle entry,
    not all XXX models provided by
    Azure are necessary.} For example, if 
    Azure only contains two models, namely
    support vector machine and boosted
    decision tree, it would also
    provide enough quality for this case.
\end{enumerate}

\begin{wrapfigure}{r}{0.12\textwidth}
  \begin{center}
    \includegraphics[width=0.12\textwidth]{fly}
  \end{center}
\end{wrapfigure}

\noindent
{\bf (Middle Tolerance Regime)}
In the regime between the low tolerance and
high tolerance regimes, we find that
{\bf there exists a level of
quality tolerances such that the extra flexibility 
provided by Azure allows it to reach the
tolerance while Amazon fails to do it}.
The figure on the right illustrates
the existence of such a regime.

\begin{table}
\scriptsize
\centering
\begin{tabular}{c|c|c|c|r|r}
\hline
Data Set & Best Azure & Best Amazon & Winning & Quality Gap & Ranking Gap (\%) \\ \hline
D-EG & C-AP & C-LR & LR &-0.01& -0.2 (No.$3 \rightarrow 2$)\\ 
D-SCH & C-BPM & C-LR & DWD &-0.01 & 0 \\ 
\hline
\hline
D-KDD1 & C-BDT & C-LR & Ensemble & 0.03  & 2.8 \\ 
D-AEA & C-DJ & C-LR & Ensemble & 0.01 & 3.6 \\ 
D-KDD2 & C-BDT & C-LR & Ensemble &0.05 & 6.4 \\ 
D-VP & C-DF & C-LR &? &0.11 & 34.6 \\ 
D-HP &  & C-LR & Ensemble& & \\ 
D-CTR &  & C-LR & Ensemble& & \\ 
D-PHY & N/A & N/A & xgboost & N/A & N/A \\ 
\hline
\end{tabular}
\caption{Low Tolerance, DWD=Distance Weighted Discrimination}
\end{table}


%Back up from EDBT submission

\begin{comment}

\begin{figure}[t]
\scriptsize
\centering
\begin{tabular}{c|r|r|r|r}
\hline
Data Set & Training Set & Testing Set & \# Features & Size (Train; Test) \\ \hline
D-SCH & 86 & 119,748 & 410 & 322KB; 489MB\\ 
D-EG & 7,395 & 3,171 & 29 & 3.2MB; 1.4MB \\ 
D-VP & 10,506 & 116,293 & 20 & 1.9MB; 21MB \\ 
D-AEA & 32,769 & 58,921 & 135 & 55MB; 98MB \\%\textcolor{blue}{135} & \textcolor{blue}{55MB};\textcolor{blue}{98MB} \\ 
D-PHY & 38,102 & 855,819 & 74 & 36MB; 860MB \\ 
D-KDD1 & 391,088 & 44,772 & 190 & 282MB; 33MB \\ 
D-KDD2 & 131,329 & 44,772 & 100 & 106MB; 37MB \\ 
%D-HP & 3,995,803 & 1,351,242 & 11 & 6.0GB; 2.0GB \\ 
%D-CTR & 40,428,967 & 4,577,464 & 49 & 14GB; 1.6GB \\ 
\hline
\end{tabular}
\caption{Statistics of Datasets}
\label{tab:stats-datasets}
%\vskip -4ex
\end{figure}

\end{comment}

\begin{comment}

\begin{figure}[t]
\tiny
\centering
\begin{tabular}{lrrrrrrr}
\hline
Model & D-SCH & D-EG &D-VP & D-AEA & D-PHY & D-KDD1 & D-KDD2  \\
\hline
 C-AP & 6 & 6 & 13 & 25 & 21 & 310 & 550 \\
 C-BPM & 9 & 13 & 14 & 241 & 114 & 3,814 & 1,450 \\
 C-BDT & 280 & 837 & 1,546 & 3,495 & 2,901 & 40,364 & 365,256 \\
 C-DF & 12 & 227 & 422 & 780 & 644 & 24,796 & 6,675 \\
 C-DJ & 130 & 690 & 2,383 & 3,413 & 3,167 & 88,044 & 9,339 \\
 C-NN & 11 & 39 & 216 & 323 & 262 & 4,465 & N/A \\
 C-SVM & 11 & 22 & 100 & 193 & 144 & 3,074 & 6,191   \\
 %C-LDSVM & 25,783 & 88,020 & 127,776\\
 C-LR & 15 & 17 & 55 & 210 & 132 & 4,455 & 7,228  \\
\hline
\end{tabular}
\caption{Total training time on Azure (in seconds) for various datasets and models.}
\label{table:performance}
%\vskip -4ex
\end{figure}

\begin{figure}[t]
\tiny
\centering
\begin{tabular}{lrrrrrrr}
\hline
            Model & D-SCH & D-EG &D-VP & D-AEA & D-PHY & D-KDD1 & D-KDD2  \\
\hline
 C-AP & 1 & 1 & 2 & 4 & 3 & 52 & 92 \\
 C-BPM & 9 & 13 & 14 & 241 & 114 & 3,814 & 1,450 \\
 C-BDT & 2 & 5 & 9 & 19 & 16 & 224 & 2,029 \\
 C-DF & 0 & 3 & 5 & 10 & 8 & 306 & 82 \\
 C-DJ & 2 & 9 & 30 & 42 & 39 & 1,087 & 115 \\
 C-NN & 0 & 2 & 9 & 13 & 11 & 186 & N/A \\
 C-SVM & 1 & 1 & 7 & 13 & 10 & 205 & 413  \\
 %C-LDSVM \\
 C-LR & 0 & 0 & 1 & 3 & 2 & 62 & 100  \\
\hline
\end{tabular}
\caption{Average training time on Azure (in seconds) for one hyper-parameter setting.}
\label{table:performance-average}
%\vskip -5ex
\end{figure}

\end{comment}

\begin{figure}
%\scriptsize
\tiny
\centering
\begin{tabular}{l|rrrrrrrr}
\toprule
\hline
Model &   C-AP & C-BPM &  C-BDT &   C-DF &   C-DJ &   C-LR &   C-NN &  C-SVM\\ %& TotalTime \\
\midrule
\hline
  D-SCH-r &      6 &     6 &    285 &     12 &    129 &     15 &     11 &     10  \\ %      474 \\
  D-PIS-r &      6 &     5 &    639 &    178 &    551 &     16 &     30 &     16   \\ %    1,441 \\
   D-EG-r &     28 &    15 &  10,165 &    260 &    530 &    145 &   3,548 &    271  \\ %    14,961 \\
   D-VP-r &     32 &     8 &   3,105 &    821 &   3,342 &    135 &    824 &    304  \\ %    8,571 \\
  D-AEA-r &     33 &    22 &  25,240 &   2,028 &   3,968 &    230 &    690 &    229   \\ %   32,442 \\
  D-SCS-r &    126 &   286 &   6,198 &   2,816 &   7,119 &    791 &   1,583 &   1,433   \\ %   20,352 \\
  D-SMR-r &  18,315 &  3,116 &    NA &  15,853 &  19,332 &    NA &    NA &    NA    \\ %  56,615 \\
  D-GMC-r &     27 &    17 &   4,146 &   4425 &  10,635 &    206 &    501 &    208  \\ %    20,164 \\
  D-HQC-r &   2,697 &   454 &  47,502 &  22,023 &    NA &  12,404 &  29,617 &  27,341   \\ %  142,039 \\
  D-KDD-r &   4,290 &   906 &    NA &  40,816 &  63,185 &  37,328 &    NA &  39,716   \\ %  186,241 \\
  D-PBV-r &  11,450 &   877 &    NA &    NA &    NA &  84,290 &    NA &    NA    \\ %  96,617 \\
  \hline
    D-SCH &      5 &     4 &    289 &     12 &    129 &     15 &     11 &      9  \\ %      474 \\
     D-EG &      7 &     5 &    852 &    229 &    696 &     17 &     38 &     20   \\ %    1,863 \\
     D-VP &     14 &     5 &   1,368 &    539 &   3,140 &     56 &    186 &     92  \\ %     5,400 \\
    D-AEA &     24 &    54 &   3,589 &    757 &   3,296 &    212 &    298 &    197   \\ %    8,426 \\
    D-PHY &     22 &    23 &   3,022 &    625 &   3,207 &    146 &    277 &    142  \\ %     7,465 \\
   D-KDD2 &    668 &   339 &    NA &   8,672 &  11,741 &   8,012 &    NA &   7,955   \\ %   37,386 \\
   D-KDD1 &   3,203 &   412 &    NA &  41,831 &    NA &  21,255 &    NA &  35,945  \\ %  102,647 \\
\bottomrule
\hline
\end{tabular}

\caption{Total training time on Azure (in seconds) for various datasets and models.}
%\label{table:performanceUpdate}
\label{table:performance}
\vskip -6ex
\end{figure}

\begin{figure}
%\scriptsize
\tiny
\centering
\begin{tabular}{l|rrrrrrrr}
\toprule
\hline
Model &  C-AP & C-BPM & C-BDT & C-DF & C-DJ & C-LR &   C-NN & C-SVM\\ %& TotalTime \\
\midrule
\hline
  D-SCH-r &     4 &     6 &     5 &    3 &    3 &    3 &      4 &     4    \\ %     34 \\
  D-PIS-r &     3 &     5 &     6 &    7 &    4 &    4 &      6 &     4    \\ %     37 \\
   D-EG-r &     7 &    15 &     9 &    6 &    4 &    4 &    247 &     4    \\ %    296 \\
   D-VP-r &     6 &     8 &     7 &    7 &    7 &    5 &     69 &     5    \\ %    114 \\
  D-AEA-r &     5 &    22 &    12 &    6 &    9 &    5 &     58 &     5    \\ %    122 \\
  D-SCS-r &    10 &   286 &    10 &   18 &   11 &    6 &    109 &     6     \\ %   456 \\
  D-SMR-r &  1,048 &  3,116 &  1,148 &   45 &   50 &  693 &    NA &   328   \\ %    6,429 \\
  D-GMC-r &     5 &    17 &    10 &   59 &   14 &    4 &     42 &     4     \\ %   156 \\
  D-HQC-r &   189 &   454 &    58 &  113 &  143 &   57 &   2,254 &    54  \\ %    3,320 \\
  D-KDD-r &   222 &   906 &   905 &   48 &   99 &  122 &    NA &    88    \\ %   2,391 \\
  D-PBV-r &   513 &   877 &   439 &  160 &  788 &  229 &    NA &   112    \\ %   3,118 \\
  \hline
    D-SCH &     4 &     4 &     5 &    3 &    3 &    4 &      4 &     4    \\ %    31 \\
    D-EG &     4 &     5 &     5 &    7 &    4 &    4 &      6 &     4     \\ %    38 \\
    D-VP &     5 &     5 &     5 &    7 &    6 &    4 &     17 &     4     \\ %    53 \\
    D-AEA &     6 &    54 &     9 &   10 &    8 &    5 &     24 &     5     \\ %   119 \\
    D-PHY &     5 &    23 &     8 &    9 &    8 &    5 &     22 &     5    \\ %     84 \\
    D-KDD1 &   183 &   412 &   161 &   41 &  117 &   73 &  46,830 &    55    \\ %  47,872 \\
    D-KDD2 &    50 &   339 &   146 &   14 &   22 &   27 &    NA &    20    \\ %   617 \\
\bottomrule
\hline
\end{tabular}

%\caption{Training time on Azure (in seconds) for the default hyper-parameter setting. }
%\label{table:performance-SingleRunUpdate}
\caption{Average training time on Azure (in seconds) for one hyper-parameter setting.}
\label{table:performance-average}
\vskip -6ex
\end{figure}


\begin{figure*}
\scriptsize
\centering
%\colorbox{red}{
\begin{tabular}{l|rr|rrrrrrrr|r}
\toprule
   Model & Leaderboard\#1 & WinningCode &         C-AP &        C-BPM &        C-BDT &         C-DF &         C-DJ &         C-LR &         C-NN &        C-SVM &          Amazon \\
\midrule
 D-SCH-r &      0.93 (1) &    0.91 (3)    &    0.88 (48) &     0.92 (3) &   0.69 (280) &   0.68 (281) &   0.82 (172) &    0.89 (30) &    0.89 (30) &    0.90 (14) &  < 0.72 (269) \\
 D-PIS-r &      0.88 (1) &             &   0.76 (127) &   0.78 (118) &    0.87 (27) &    0.86 (62) &    0.87 (48) &   0.78 (118) &   0.80 (114) &   0.77 (120) &    0.86 (66) \\
  D-EG-r &      0.89 (1) &   0.89 (4)    &   0.86 (388) &   0.86 (381) &   0.86 (374) &   0.86 (382) &   0.86 (388) &   0.86 (388) &   0.86 (388) &   0.85 (400) &    NA (NA) \\
  D-VP-r &      0.86 (1) &   0.86 (1)   &  0.63 (1105) &  0.64 (1083) &   0.69 (840) &  0.63 (1100) &  0.60 (1137) &   0.67 (928) &  0.66 (1023) &  0.57 (1157) &   0.66 (989) \\
 D-AEA-r &      0.92 (1) &   0.92 (2)   &   0.87 (834) &   0.84 (932) &   0.87 (802) &   0.86 (889) &  0.79 (1049) &   0.88 (737) &   0.87 (798) &   0.86 (869) &   0.85 (901) \\
 D-SCS-r &      0.83 (1) &  0.83 (3)   &  0.75 (4128) &  0.77 (4038) &  0.82 (3084) &  0.82 (3432) &  0.82 (3240) &  0.78 (4019) &  0.79 (3916) &  0.71 (4302) &  0.81 (3691) \\
 D-SMR-r &      0.80 (1) &             &  0.74 (1826) &  0.70 (1898) &    NA (NA) &  0.73 (1842) &  0.71 (1888) &    NA (NA) &    NA (NA) &    NA (NA) &    NA (NA) \\
 D-GMC-r &      0.87 (1) &             &   0.74 (810) &   0.70 (820) &   0.87 (137) &   0.86 (505) &   0.87 (139) &   0.70 (837) &   0.83 (713) &   0.81 (750) &   0.86 (544) \\
 D-HQC-r &      0.97 (1) &             &  0.94 (1431) &  0.93 (1476) &   0.97 (977) &  0.96 (1206) &    NA (NA) &  0.94 (1429) &  0.95 (1335) &  0.94 (1463) &  0.96 (1294) \\
 D-KDD-r &      0.68 (1) &    0.67 (2)   &   0.59 (130) &   0.55 (314) &    NA (NA) &   0.56 (297) &   0.54 (373) &    0.60 (77) &    NA (NA) &   0.54 (363) &   0.58 (152) \\
 D-PBV-r &      1.00 (1) &             &  0.95 (1651) &  0.98 (1498) &    NA (NA) &    NA (NA) &    NA (NA) &  0.97 (1529) &    NA (NA) &    NA (NA) &  0.96 (1612) \\
 
 \midrule
 
   D-SCH &      0.93 (1) &    0.91 (3)    &    0.88 (48) &     0.92 (3) &   0.69 (280) &   0.68 (281) &   0.82 (172) &    0.89 (30) &    0.89 (30) &    0.90 (14) &  < 0.72 (269) \\
    D-EG &      0.89 (1) &   0.89 (4)  &     0.89 (2) &     0.89 (3) &    0.88 (54) &   0.88 (278) &   0.88 (291) &     0.89 (2) &     0.89 (7) &     0.89 (2) &   0.88 (327) \\
    D-VP &      0.86 (1) &  0.86 (1)   &   0.66 (987) &  0.56 (1161) &   0.74 (488) &   0.72 (601) &   0.73 (546) &   0.71 (694) &   0.72 (616) &   0.72 (586) &   0.76 (392) \\
   D-AEA &      0.92 (1) &  0.92 (2)   &    0.91 (75) &    0.91 (94) &    0.92 (29) &   0.90 (147) &    0.91 (63) &    0.91 (72) &    0.91 (72) &   0.90 (401) &   0.90 (189) \\
   D-PHY &      1.00 (1) &  1.00 (2)   &    NA (NA) &    NA (NA) &    NA (NA) &    NA (NA) &    NA (NA) &    NA (NA) &    NA (NA) &    NA (NA) &    NA (NA) \\
  D-KDD2 &      0.68 (1) &  0.67 (2)   &   0.57 (200) &   0.54 (372) &    NA (NA) &    0.60 (74) &    0.59 (92) &   0.57 (206) &    NA (NA) &   0.57 (245) &    0.61 (57) \\
  D-KDD1 &      0.68 (1) &  0.67 (2)   &    0.62 (43) &    0.60 (79) &    NA (NA) &    0.60 (81) &    NA (NA) &   0.59 (135) &    NA (NA) &   0.59 (103) &    0.63 (27) \\
\bottomrule
\end{tabular}

%}
% \begin{tabular}{lllllllll}
% \hline
%           & Model & D-SCH (313) & D-EG (625) & D-VP (1306) & D-AEA (1687) & D-PHY (673) & D-KDD1 (472) & D-KDD2 (472) \\
% \hline
% Winning   &  & 0.91 (3) & 0.89 (4) & 0.86 (1) & 0.92 (2) & 1.00 (2) & \multicolumn{2}{c}{0.67 (2)}    \\
% \hline
% \multirow{8}{3em}{Azure} 
% & C-AP & 0.88 (37) & 0.89 (2) & 0.65 (1046) & 0.91 (75) & N/A (N/A) & 0.65 (12) & 0.58 (192) \\
% & C-BPM & 0.92 (3) & 0.89 (3) & 0.70 (734) & 0.91 (94) & N/A (N/A) & 0.64 (25) & 0.51 (399) \\
% & C-BDT & 0.69 (279) & 0.88 (54) & 0.76 (408) & 0.92 (29) & N/A (N/A) & 0.64 (26) & 0.62 (33) \\
% & C-DF & 0.68 (281) & 0.88 (278) & 0.74 (473) & 0.90 (147) & N/A (N/A) & 0.62 (40) & 0.61 (53)  \\
% & C-DJ & 0.82 (165) & 0.88 (291) & 0.72 (568) & 0.91 (63) & N/A (N/A) & 0.64 (25) & 0.60 (72)  \\
% & C-NN & 0.88 (30) & 0.89 (4) & 0.74 (496) & 0.91 (72) & N/A (N/A) & 0.60 (68) & N/A (N/A) \\
% & C-SVM & 0.90 (8) & 0.89 (2) & 0.72 (613) & 0.90 (401)  & N/A (N/A) & 0.64 (20) & 0.57 (206)  \\
% %& C-LDSVM & 0.88 (37) & 0.88(259) & 0.67 (972) & \\
% & C-LR & 0.89 (22) & 0.89 (2) & 0.71 (648) & 0.91 (72) & N/A (N/A) & 0.65 (12) & 0.58 (198)  \\
% \hline
% Amazon & C-LR & 0.74 (264) & 0.88 (326) & 0.68 (923) & 0.90 (361) & N/A (N/A) & 0.63 (29) & 0.60 (65) \\
% \hline
% \end{tabular}
\caption{Area under curve (AUC) and rank on the private leader board of Kaggle for various datasets and models. The winning code of KDD is an ensemble of the classifiers trained from both D-KDD1 and D-KDD2.}
\label{tab:quality}
\vskip -2ex
\end{figure*}


==> backup.tex <==
%\vspace{-1em}
\section{Backup}

\paragraph*{Premier of Clouds APIs} 

\vspace{-1em}
\paragraph*{Summary of Insights} Our
study is organized with the following
structure. We mainly focus on three aspects
of machine learning clouds: (1) {\em Is
the set of machine learning models
enough?} (2) {\em Is the performance of 
training enough?} and (3) {\em Is the hyperparameter
tuning support enough?} For each 
level of error tolerances and budget
of time and money, we discuss 
each of these three questions for
each of the two machine learning. In
this paper, we fully studied this 
``cross product'' and highlight some
interesting insights here.\\

\vspace{-0.5em}
\noindent
{\bf (Low Tolerance Regime)} 
This regime corresponds to
the case when the error tolerance from the user
is low --- for example, when users can only be
satisfied by winning the Kaggle competition
or being ranked among the top 1\%.
Our study reveals the following:
\begin{enumerate}
    \vspace{-0.25em}
    \item {\bf Even with the same features
    engineered by the winning Kaggle entry, 
    neither Azure nor Amazon is able to meet  
    the tolerance for {\em all} datasets.}
    The fundamental reason is that both clouds
    miss ensemble-based models in their API.
    \item {\bf ?????}
\end{enumerate}

\noindent
{\bf (High Tolerance Regime)}
This regime corresponds to
the case when the error tolerance from the user
is high --- for example, when users are 
happy with suboptimal quality that is only
up to 5 points lower than the winning Kaggle
entry or being ranked among the top 10\%.
Our study reveals the following:
\begin{enumerate}
    \vspace{-0.25em}
    \item {\bf With the same features
    engineered by the winning Kaggle entry,
    both Azure and Amazon are able to meet
    the tolerance for {\em most} datasets.}
    For example, the default setting of Amazon 
    can already provide enough quality for this case.
    \vspace{-0.25em}
    \item {\bf With the same features
    engineered by the winning Kaggle entry,
    not all XXX models provided by
    Azure are necessary.} For example, if 
    Azure only contains two models, namely
    support vector machine and boosted
    decision tree, it would also
    provide enough quality for this case.
\end{enumerate}

\begin{wrapfigure}{r}{0.12\textwidth}
  \begin{center}
    \includegraphics[width=0.12\textwidth]{fly}
  \end{center}
\end{wrapfigure}

\noindent
{\bf (Middle Tolerance Regime)}
In the regime between the low tolerance and
high tolerance regimes, we find that
{\bf there exists a level of
quality tolerances such that the extra flexibility 
provided by Azure allows it to reach the
tolerance while Amazon fails to do it}.
The figure on the right illustrates
the existence of such a regime.

\begin{table}
\scriptsize
\centering
\begin{tabular}{c|c|c|c|r|r}
\hline
Data Set & Best Azure & Best Amazon & Winning & Quality Gap & Ranking Gap (\%) \\ \hline
D-EG & C-AP & C-LR & LR &-0.01& -0.2 (No.$3 \rightarrow 2$)\\ 
D-SCH & C-BPM & C-LR & DWD &-0.01 & 0 \\ 
\hline
\hline
D-KDD1 & C-BDT & C-LR & Ensemble & 0.03  & 2.8 \\ 
D-AEA & C-DJ & C-LR & Ensemble & 0.01 & 3.6 \\ 
D-KDD2 & C-BDT & C-LR & Ensemble &0.05 & 6.4 \\ 
D-VP & C-DF & C-LR &? &0.11 & 34.6 \\ 
D-HP &  & C-LR & Ensemble& & \\ 
D-CTR &  & C-LR & Ensemble& & \\ 
D-PHY & N/A & N/A & xgboost & N/A & N/A \\ 
\hline
\end{tabular}
\caption{Low Tolerance, DWD=Distance Weighted Discrimination}
\end{table}


%Back up from EDBT submission

\begin{comment}

\begin{figure}[t]
\scriptsize
\centering
\begin{tabular}{c|r|r|r|r}
\hline
Data Set & Training Set & Testing Set & \# Features & Size (Train; Test) \\ \hline
D-SCH & 86 & 119,748 & 410 & 322KB; 489MB\\ 
D-EG & 7,395 & 3,171 & 29 & 3.2MB; 1.4MB \\ 
D-VP & 10,506 & 116,293 & 20 & 1.9MB; 21MB \\ 
D-AEA & 32,769 & 58,921 & 135 & 55MB; 98MB \\%\textcolor{blue}{135} & \textcolor{blue}{55MB};\textcolor{blue}{98MB} \\ 
D-PHY & 38,102 & 855,819 & 74 & 36MB; 860MB \\ 
D-KDD1 & 391,088 & 44,772 & 190 & 282MB; 33MB \\ 
D-KDD2 & 131,329 & 44,772 & 100 & 106MB; 37MB \\ 
%D-HP & 3,995,803 & 1,351,242 & 11 & 6.0GB; 2.0GB \\ 
%D-CTR & 40,428,967 & 4,577,464 & 49 & 14GB; 1.6GB \\ 
\hline
\end{tabular}
\caption{Statistics of Datasets}
\label{tab:stats-datasets}
%\vskip -4ex
\end{figure}

\end{comment}

\begin{comment}

\begin{figure}[t]
\tiny
\centering
\begin{tabular}{lrrrrrrr}
\hline
Model & D-SCH & D-EG &D-VP & D-AEA & D-PHY & D-KDD1 & D-KDD2  \\
\hline
 C-AP & 6 & 6 & 13 & 25 & 21 & 310 & 550 \\
 C-BPM & 9 & 13 & 14 & 241 & 114 & 3,814 & 1,450 \\
 C-BDT & 280 & 837 & 1,546 & 3,495 & 2,901 & 40,364 & 365,256 \\
 C-DF & 12 & 227 & 422 & 780 & 644 & 24,796 & 6,675 \\
 C-DJ & 130 & 690 & 2,383 & 3,413 & 3,167 & 88,044 & 9,339 \\
 C-NN & 11 & 39 & 216 & 323 & 262 & 4,465 & N/A \\
 C-SVM & 11 & 22 & 100 & 193 & 144 & 3,074 & 6,191   \\
 %C-LDSVM & 25,783 & 88,020 & 127,776\\
 C-LR & 15 & 17 & 55 & 210 & 132 & 4,455 & 7,228  \\
\hline
\end{tabular}
\caption{Total training time on Azure (in seconds) for various datasets and models.}
\label{table:performance}
%\vskip -4ex
\end{figure}

\begin{figure}[t]
\tiny
\centering
\begin{tabular}{lrrrrrrr}
\hline
            Model & D-SCH & D-EG &D-VP & D-AEA & D-PHY & D-KDD1 & D-KDD2  \\
\hline
 C-AP & 1 & 1 & 2 & 4 & 3 & 52 & 92 \\
 C-BPM & 9 & 13 & 14 & 241 & 114 & 3,814 & 1,450 \\
 C-BDT & 2 & 5 & 9 & 19 & 16 & 224 & 2,029 \\
 C-DF & 0 & 3 & 5 & 10 & 8 & 306 & 82 \\
 C-DJ & 2 & 9 & 30 & 42 & 39 & 1,087 & 115 \\
 C-NN & 0 & 2 & 9 & 13 & 11 & 186 & N/A \\
 C-SVM & 1 & 1 & 7 & 13 & 10 & 205 & 413  \\
 %C-LDSVM \\
 C-LR & 0 & 0 & 1 & 3 & 2 & 62 & 100  \\
\hline
\end{tabular}
\caption{Average training time on Azure (in seconds) for one hyper-parameter setting.}
\label{table:performance-average}
%\vskip -5ex
\end{figure}

\end{comment}

\begin{figure}
%\scriptsize
\tiny
\centering
\begin{tabular}{l|rrrrrrrr}
\toprule
\hline
Model &   C-AP & C-BPM &  C-BDT &   C-DF &   C-DJ &   C-LR &   C-NN &  C-SVM\\ %& TotalTime \\
\midrule
\hline
  D-SCH-r &      6 &     6 &    285 &     12 &    129 &     15 &     11 &     10  \\ %      474 \\
  D-PIS-r &      6 &     5 &    639 &    178 &    551 &     16 &     30 &     16   \\ %    1,441 \\
   D-EG-r &     28 &    15 &  10,165 &    260 &    530 &    145 &   3,548 &    271  \\ %    14,961 \\
   D-VP-r &     32 &     8 &   3,105 &    821 &   3,342 &    135 &    824 &    304  \\ %    8,571 \\
  D-AEA-r &     33 &    22 &  25,240 &   2,028 &   3,968 &    230 &    690 &    229   \\ %   32,442 \\
  D-SCS-r &    126 &   286 &   6,198 &   2,816 &   7,119 &    791 &   1,583 &   1,433   \\ %   20,352 \\
  D-SMR-r &  18,315 &  3,116 &    NA &  15,853 &  19,332 &    NA &    NA &    NA    \\ %  56,615 \\
  D-GMC-r &     27 &    17 &   4,146 &   4425 &  10,635 &    206 &    501 &    208  \\ %    20,164 \\
  D-HQC-r &   2,697 &   454 &  47,502 &  22,023 &    NA &  12,404 &  29,617 &  27,341   \\ %  142,039 \\
  D-KDD-r &   4,290 &   906 &    NA &  40,816 &  63,185 &  37,328 &    NA &  39,716   \\ %  186,241 \\
  D-PBV-r &  11,450 &   877 &    NA &    NA &    NA &  84,290 &    NA &    NA    \\ %  96,617 \\
  \hline
    D-SCH &      5 &     4 &    289 &     12 &    129 &     15 &     11 &      9  \\ %      474 \\
     D-EG &      7 &     5 &    852 &    229 &    696 &     17 &     38 &     20   \\ %    1,863 \\
     D-VP &     14 &     5 &   1,368 &    539 &   3,140 &     56 &    186 &     92  \\ %     5,400 \\
    D-AEA &     24 &    54 &   3,589 &    757 &   3,296 &    212 &    298 &    197   \\ %    8,426 \\
    D-PHY &     22 &    23 &   3,022 &    625 &   3,207 &    146 &    277 &    142  \\ %     7,465 \\
   D-KDD2 &    668 &   339 &    NA &   8,672 &  11,741 &   8,012 &    NA &   7,955   \\ %   37,386 \\
   D-KDD1 &   3,203 &   412 &    NA &  41,831 &    NA &  21,255 &    NA &  35,945  \\ %  102,647 \\
\bottomrule
\hline
\end{tabular}

\caption{Total training time on Azure (in seconds) for various datasets and models.}
%\label{table:performanceUpdate}
\label{table:performance}
\vskip -6ex
\end{figure}

\begin{figure}
%\scriptsize
\tiny
\centering
\begin{tabular}{l|rrrrrrrr}
\toprule
\hline
Model &  C-AP & C-BPM & C-BDT & C-DF & C-DJ & C-LR &   C-NN & C-SVM\\ %& TotalTime \\
\midrule
\hline
  D-SCH-r &     4 &     6 &     5 &    3 &    3 &    3 &      4 &     4    \\ %     34 \\
  D-PIS-r &     3 &     5 &     6 &    7 &    4 &    4 &      6 &     4    \\ %     37 \\
   D-EG-r &     7 &    15 &     9 &    6 &    4 &    4 &    247 &     4    \\ %    296 \\
   D-VP-r &     6 &     8 &     7 &    7 &    7 &    5 &     69 &     5    \\ %    114 \\
  D-AEA-r &     5 &    22 &    12 &    6 &    9 &    5 &     58 &     5    \\ %    122 \\
  D-SCS-r &    10 &   286 &    10 &   18 &   11 &    6 &    109 &     6     \\ %   456 \\
  D-SMR-r &  1,048 &  3,116 &  1,148 &   45 &   50 &  693 &    NA &   328   \\ %    6,429 \\
  D-GMC-r &     5 &    17 &    10 &   59 &   14 &    4 &     42 &     4     \\ %   156 \\
  D-HQC-r &   189 &   454 &    58 &  113 &  143 &   57 &   2,254 &    54  \\ %    3,320 \\
  D-KDD-r &   222 &   906 &   905 &   48 &   99 &  122 &    NA &    88    \\ %   2,391 \\
  D-PBV-r &   513 &   877 &   439 &  160 &  788 &  229 &    NA &   112    \\ %   3,118 \\
  \hline
    D-SCH &     4 &     4 &     5 &    3 &    3 &    4 &      4 &     4    \\ %    31 \\
    D-EG &     4 &     5 &     5 &    7 &    4 &    4 &      6 &     4     \\ %    38 \\
    D-VP &     5 &     5 &     5 &    7 &    6 &    4 &     17 &     4     \\ %    53 \\
    D-AEA &     6 &    54 &     9 &   10 &    8 &    5 &     24 &     5     \\ %   119 \\
    D-PHY &     5 &    23 &     8 &    9 &    8 &    5 &     22 &     5    \\ %     84 \\
    D-KDD1 &   183 &   412 &   161 &   41 &  117 &   73 &  46,830 &    55    \\ %  47,872 \\
    D-KDD2 &    50 &   339 &   146 &   14 &   22 &   27 &    NA &    20    \\ %   617 \\
\bottomrule
\hline
\end{tabular}

%\caption{Training time on Azure (in seconds) for the default hyper-parameter setting. }
%\label{table:performance-SingleRunUpdate}
\caption{Average training time on Azure (in seconds) for one hyper-parameter setting.}
\label{table:performance-average}
\vskip -6ex
\end{figure}


\begin{figure*}
\scriptsize
\centering
%\colorbox{red}{
\begin{tabular}{l|rr|rrrrrrrr|r}
\toprule
   Model & Leaderboard\#1 & WinningCode &         C-AP &        C-BPM &        C-BDT &         C-DF &         C-DJ &         C-LR &         C-NN &        C-SVM &          Amazon \\
\midrule
 D-SCH-r &      0.93 (1) &    0.91 (3)    &    0.88 (48) &     0.92 (3) &   0.69 (280) &   0.68 (281) &   0.82 (172) &    0.89 (30) &    0.89 (30) &    0.90 (14) &  < 0.72 (269) \\
 D-PIS-r &      0.88 (1) &             &   0.76 (127) &   0.78 (118) &    0.87 (27) &    0.86 (62) &    0.87 (48) &   0.78 (118) &   0.80 (114) &   0.77 (120) &    0.86 (66) \\
  D-EG-r &      0.89 (1) &   0.89 (4)    &   0.86 (388) &   0.86 (381) &   0.86 (374) &   0.86 (382) &   0.86 (388) &   0.86 (388) &   0.86 (388) &   0.85 (400) &    NA (NA) \\
  D-VP-r &      0.86 (1) &   0.86 (1)   &  0.63 (1105) &  0.64 (1083) &   0.69 (840) &  0.63 (1100) &  0.60 (1137) &   0.67 (928) &  0.66 (1023) &  0.57 (1157) &   0.66 (989) \\
 D-AEA-r &      0.92 (1) &   0.92 (2)   &   0.87 (834) &   0.84 (932) &   0.87 (802) &   0.86 (889) &  0.79 (1049) &   0.88 (737) &   0.87 (798) &   0.86 (869) &   0.85 (901) \\
 D-SCS-r &      0.83 (1) &  0.83 (3)   &  0.75 (4128) &  0.77 (4038) &  0.82 (3084) &  0.82 (3432) &  0.82 (3240) &  0.78 (4019) &  0.79 (3916) &  0.71 (4302) &  0.81 (3691) \\
 D-SMR-r &      0.80 (1) &             &  0.74 (1826) &  0.70 (1898) &    NA (NA) &  0.73 (1842) &  0.71 (1888) &    NA (NA) &    NA (NA) &    NA (NA) &    NA (NA) \\
 D-GMC-r &      0.87 (1) &             &   0.74 (810) &   0.70 (820) &   0.87 (137) &   0.86 (505) &   0.87 (139) &   0.70 (837) &   0.83 (713) &   0.81 (750) &   0.86 (544) \\
 D-HQC-r &      0.97 (1) &             &  0.94 (1431) &  0.93 (1476) &   0.97 (977) &  0.96 (1206) &    NA (NA) &  0.94 (1429) &  0.95 (1335) &  0.94 (1463) &  0.96 (1294) \\
 D-KDD-r &      0.68 (1) &    0.67 (2)   &   0.59 (130) &   0.55 (314) &    NA (NA) &   0.56 (297) &   0.54 (373) &    0.60 (77) &    NA (NA) &   0.54 (363) &   0.58 (152) \\
 D-PBV-r &      1.00 (1) &             &  0.95 (1651) &  0.98 (1498) &    NA (NA) &    NA (NA) &    NA (NA) &  0.97 (1529) &    NA (NA) &    NA (NA) &  0.96 (1612) \\
 
 \midrule
 
   D-SCH &      0.93 (1) &    0.91 (3)    &    0.88 (48) &     0.92 (3) &   0.69 (280) &   0.68 (281) &   0.82 (172) &    0.89 (30) &    0.89 (30) &    0.90 (14) &  < 0.72 (269) \\
    D-EG &      0.89 (1) &   0.89 (4)  &     0.89 (2) &     0.89 (3) &    0.88 (54) &   0.88 (278) &   0.88 (291) &     0.89 (2) &     0.89 (7) &     0.89 (2) &   0.88 (327) \\
    D-VP &      0.86 (1) &  0.86 (1)   &   0.66 (987) &  0.56 (1161) &   0.74 (488) &   0.72 (601) &   0.73 (546) &   0.71 (694) &   0.72 (616) &   0.72 (586) &   0.76 (392) \\
   D-AEA &      0.92 (1) &  0.92 (2)   &    0.91 (75) &    0.91 (94) &    0.92 (29) &   0.90 (147) &    0.91 (63) &    0.91 (72) &    0.91 (72) &   0.90 (401) &   0.90 (189) \\
   D-PHY &      1.00 (1) &  1.00 (2)   &    NA (NA) &    NA (NA) &    NA (NA) &    NA (NA) &    NA (NA) &    NA (NA) &    NA (NA) &    NA (NA) &    NA (NA) \\
  D-KDD2 &      0.68 (1) &  0.67 (2)   &   0.57 (200) &   0.54 (372) &    NA (NA) &    0.60 (74) &    0.59 (92) &   0.57 (206) &    NA (NA) &   0.57 (245) &    0.61 (57) \\
  D-KDD1 &      0.68 (1) &  0.67 (2)   &    0.62 (43) &    0.60 (79) &    NA (NA) &    0.60 (81) &    NA (NA) &   0.59 (135) &    NA (NA) &   0.59 (103) &    0.63 (27) \\
\bottomrule
\end{tabular}

%}
% \begin{tabular}{lllllllll}
% \hline
%           & Model & D-SCH (313) & D-EG (625) & D-VP (1306) & D-AEA (1687) & D-PHY (673) & D-KDD1 (472) & D-KDD2 (472) \\
% \hline
% Winning   &  & 0.91 (3) & 0.89 (4) & 0.86 (1) & 0.92 (2) & 1.00 (2) & \multicolumn{2}{c}{0.67 (2)}    \\
% \hline
% \multirow{8}{3em}{Azure} 
% & C-AP & 0.88 (37) & 0.89 (2) & 0.65 (1046) & 0.91 (75) & N/A (N/A) & 0.65 (12) & 0.58 (192) \\
% & C-BPM & 0.92 (3) & 0.89 (3) & 0.70 (734) & 0.91 (94) & N/A (N/A) & 0.64 (25) & 0.51 (399) \\
% & C-BDT & 0.69 (279) & 0.88 (54) & 0.76 (408) & 0.92 (29) & N/A (N/A) & 0.64 (26) & 0.62 (33) \\
% & C-DF & 0.68 (281) & 0.88 (278) & 0.74 (473) & 0.90 (147) & N/A (N/A) & 0.62 (40) & 0.61 (53)  \\
% & C-DJ & 0.82 (165) & 0.88 (291) & 0.72 (568) & 0.91 (63) & N/A (N/A) & 0.64 (25) & 0.60 (72)  \\
% & C-NN & 0.88 (30) & 0.89 (4) & 0.74 (496) & 0.91 (72) & N/A (N/A) & 0.60 (68) & N/A (N/A) \\
% & C-SVM & 0.90 (8) & 0.89 (2) & 0.72 (613) & 0.90 (401)  & N/A (N/A) & 0.64 (20) & 0.57 (206)  \\
% %& C-LDSVM & 0.88 (37) & 0.88(259) & 0.67 (972) & \\
% & C-LR & 0.89 (22) & 0.89 (2) & 0.71 (648) & 0.91 (72) & N/A (N/A) & 0.65 (12) & 0.58 (198)  \\
% \hline
% Amazon & C-LR & 0.74 (264) & 0.88 (326) & 0.68 (923) & 0.90 (361) & N/A (N/A) & 0.63 (29) & 0.60 (65) \\
% \hline
% \end{tabular}
\caption{Area under curve (AUC) and rank on the private leader board of Kaggle for various datasets and models. The winning code of KDD is an ensemble of the classifiers trained from both D-KDD1 and D-KDD2.}
\label{tab:quality}
\vskip -2ex
\end{figure*}

